LHAPDF6: parton density access in the LHC precision era

The Fortran LHAPDF library has been a long-term workhorse in particle physics, providing standardised access to parton density functions for experimental and phenomenological purposes alike, following on from the venerable PDFLIB package. During Run 1 of the LHC, however, several fundamental limitations in LHAPDF's design have became deeply problematic, restricting the usability of the library for important physics-study procedures and providing dangerous avenues by which to silently obtain incorrect results. In this paper we present the LHAPDF 6 library, a ground-up re-engineering of the PDFLIB/LHAPDF paradigm for PDF access which removes all limits on use of concurrent PDF sets, massively reduces static memory requirements, offers improved CPU performance, and fixes fundamental bugs in multi-set access to PDF metadata. The new design, restricted for now to interpolated PDFs, uses centralised numerical routines and a powerful cascading metadata system to decouple software releases from provision of new PDF data and allow completely general parton content. More than 200 PDF sets have been migrated from LHAPDF 5 to the new universal data format, via a stringent quality control procedure. LHAPDF 6 is supported by many Monte Carlo generators and other physics programs, in some cases via a full set of compatibility routines, and is recommended for the demanding PDF access needs of LHC Run 2 and beyond.

==> preamble.tex <==
%auto-ignore

\usepackage[a4paper]{geometry}
\usepackage{a4wide}
\usepackage{xcolor,graphicx}
%\usepackage{tikz,todonotes}
\usepackage{hyperref}
\usepackage{xspace}
\usepackage{relsize}
\usepackage[update,prepend]{epstopdf}
\usepackage{listings}
\usepackage{amsmath}
\usepackage{cancel}
\usepackage{url}
\usepackage{microtype}
\usepackage{booktabs}
\usepackage{bm}
% \usepackage{underscore}
% \usepackage{mathpazo}
% \usepackage[latin1]{inputenc}
% \usepackage[english]{babel}
% \usepackage[T1]{fontenc}

\frenchspacing

\newcommand{\img}[2][1.0]{\includegraphics[width=#1\textwidth]{#2}\xspace}
\newcommand{\bold}[1]{\textbf{#1}}

% \newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\red}[1]{\textcolor{red!90!black}{#1}}
\newcommand{\green}[1]{\textcolor{green!70!black}{#1}}
\newcommand{\blue}[1]{\textcolor{blue!80!white}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\grey}[1]{\textcolor{gray}{#1}}

\newcommand{\eV}{\ensuremath{\text{e}\mspace{-0.8mu}\text{V}\xspace}}
\newcommand{\MeV}{\ensuremath{\text{M\eV}}\xspace}
\newcommand{\GeV}{\ensuremath{\text{G\eV}}\xspace}
\newcommand{\TeV}{\ensuremath{\text{T\eV}}\xspace}

\renewcommand{\d}[1]{\ensuremath{\mathrm{d}#1}\xspace}
\newcommand{\pt}{\ensuremath{p_T}\xspace}
\newcommand{\qsq}{\ensuremath{Q^2}\xspace}
\newcommand{\xf}{\ensuremath{xf}\xspace}
\newcommand{\xq}{\ensuremath{(x,Q)}\xspace}
\newcommand{\xqsq}{\ensuremath{(x,Q^2)}\xspace}
\newcommand{\fxq}{\ensuremath{f\xq}\xspace}
\newcommand{\fxqsq}{\ensuremath{f\xqsq}\xspace}
\newcommand{\xfxq}{\ensuremath{x\fxq}\xspace}
\newcommand{\xfxqsq}{\ensuremath{x\fxqsq}\xspace}
\newcommand{\alphaS}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\Fortran}{\textsc{Fortran}\xspace}

\makeatletter
\newcommand{\kbd}[1]{{\smaller{\texttt{#1}}}}
\newcommand{\code}[1]{\kbd{#1}\xspace}
\newcommand{\To}{\ensuremath{\Rightarrow}\xspace}
\g@addto@macro\bfseries{\boldmath}
\makeatother

\lstset{language=c++}
% \lstset{basicstyle=\color{blue!50!green!80!black}\ttfamily\bfseries\small\smaller}
\lstset{commentstyle=\textit}

